Cyber Physical Aquaponic System (CyPhA): a CPS Testbed

Aquaponics system promises a sustainable urban development and food production by combining vegetable and fish farming in a single water loop. However, traditional aquaponics suffers from a significant amount of manual intervention with regard to decision-making in the water circulation and water quality control. In this work, we design, build and deploy a laboratory-scale real aquaponics system by considering this system as a cyber physical system, and we call it as Cyber Physical Aquaponics (CyPhA) system. The design of our CyPhA system has five stages, Stage-1 contains a vertical vegetable farming unit, Stage-2 contains fish farming unit, Stage-3 contains natural nitrification system, Stage-4 contains bio-filtration system and Stage-5 contains water accumulation and release system. Water transfer from one stage to the next is done using water pumps, and oxygen mixing in the water in any stage is achieved using aeration pumps. CyPhA system uses sensors for pH, dissolved oxygen (DO), total dissolved solid (TDS), water temperature, air temperature and humidity. A critical level of any of the water parameters in any stage is indicated using a LED-based alert indicator. Sensor data and actuator control commands among the stagewise edge devices and the CyPhA Controller are exchanged over Message Queue Telemetry Transport (MQTT) protocol. Overall, CyPhA system is housed within an area of about 80 sq. ft. We have been successfully operating CyPhA system for the last 75 days and maintaining a good quality of water for both fish and vegetable farming units.

==> figure_statemachine.tex <==
\usepackage{tikz}
\usetikzlibrary{arrows,automata,positioning}

\begin{document}
   
\begin{tikzpicture}

  \node[state,initial]   (s)                      {$s$};
  \node[state,accepting] (q_1) [below left of=s]  {$q_1$};
  \node[state]           (q_2) [below of=q_1]     {$q_2$};
  \node[state,accepting] (r_1) [below right of=s] {$r_1$};
  \node[state]           (r_2) [below of=r_1]     {$r_2$};

  \path[->]
  (s)   edge              node {a} (q_1)
        edge              node {b} (r_1)
  (q_1) edge [loop left]  node {a} (   )
        edge [bend left]  node {b} (q_2)
  (q_2) edge [loop left]  node {b} (   )
        edge [bend left]  node {a} (q_1)
  (r_1) edge [loop right] node {b} (   )
        edge [bend left]  node {a} (r_2)
  (r_2) edge [loop right] node {a} (   )
        edge [bend left]  node {b} (r_1);
\end{tikzpicture}
\end{document}
\end{document}
